Two-step estimation in linear regressions with adaptive learning

Weak consistency and asymptotic normality of the ordinary least-squares estimator in a linear regression with adaptive learning is derived when the crucial, so-called, `gain' parameter is estimated in a first step by nonlinear least squares from an auxiliary model. The singular limiting distribution of the two-step estimator is normal and in general affected by the sampling uncertainty from the first step. However, this `generated-regressor' issue disappears for certain parameter combinations.

==> nls_aux_old.tex <==
\subsection{Auxiliary Lemmata}

\renewcommand{\thelemma}{A.1}
\begin{lemma}\label{lemma_aux2} Suppose \(\{v_t,\mathcal{H}_t\}_{t \geq 1}\) forms a martingale difference sequences with \(\Ex[v_t^2 \mid \mathcal{H}_{t-1}] = \sigma_v^2 \in (0,\infty)\) and \(a_{t-1}(\theta)\) is adapted to \(\mathcal{H}_{t-1}\) uniformly in \(\theta \inn [\ubtheta,\btheta]\). Then, for any \(m \in \mathbb{N}_+\)
\begin{align}
\normalfont\sumt^n \ssupt (\ma_{t-1}(\theta))^2= \,&  O_p(\ln\,n) \tag{\textit{i}} \\
\normalfont\sumt^n \ssupt (\ma_{t-1}(\theta))^2 v_t^2 = \,&  O_p(\ln\,n) \tag{\textit{ii}} \\
\normalfont\ssupt \bigg\vert\sumt^n \ma_{t-1}(\theta)v_t \bigg\vert = \,&  O_p(\ln\,n). \tag{\textit{iii}}
\end{align}
\end{lemma}

\renewcommand{\thelemma}{A.2}
\begin{lemma}\label{lemma_aux3}
For any \(\theta \in [\ubtheta,\btheta]\), one has \textnormal{($pointwise$)}
\begin{align}
\lni \sumt^n a_t^{\st 2}(\theta) = \,& \sigma_\eps^2 \frac{\theta^2}{2\theta-1}\bigg[1+2\frac{\theta_0(1-c_0)(\theta_0(1+c_0)-1)}{(2c_0\theta_0-1)(c_0\theta_0+\theta-1)}\bigg]+ o_p(1) \tag{\textit{i}} \\
\lni \sumt^n a_t^{\st}a_t^{\st}(\theta) = \,& \sigma_\eps^2 \frac{\theta\theta_0((1 + c_0)\theta_0-1)}{(c_0\theta_0+\theta-1)(2c_0\theta_0-1)}+ o_p(1), \tag{\textit{ii}} 
\end{align}
where \(c_0 = 1-\beta_0\). Moreover,
\begin{align}
\lni \sumt^n \da_t^2 = \,& \sigma_{\da}^2+ o_p(1) \tag{\textit{iii}}\\
\lni \sumt^n a_t^\st \da_t = \,&  \left(\frac{\sigma_a}{\theta_0}\right)^2\frac{\theta_0(1-c_0\theta_0)}{1-\theta_0(1+c_0)} + o_p(1).  \tag{\textit{iv}} 
\end{align}
\end{lemma}

\renewcommand{\thelemma}{A.3}
\begin{lemma}\label{lemma_aux4} For any \(m \in \mathbb{N}_+\) and \(r \in \{2,4\}\)
\[
\Ex^{1/r}\left[(\ma_n(\theta))^r\right] = O(n^{1/2}).
\]
\end{lemma}

\renewcommand{\thelemma}{A.4} 
\begin{lemma}\label{lemma_aux5}  
\(
\Ex\big[\ssupt\ssup\limits_{\mathfrak{a}\inn\mathbb{R}}|Q_n(\theta,\mathfrak{a})-Q_n^\dagger(\theta)|\big] = O(1).
\)
\end{lemma}


\renewcommand{\thelemma}{A.5} 
\begin{lemma}\label{lemma_aux1} 
For any \(m \in \mathbb{N}_+\) and \(r \in \{1,2\}\)
\begin{align}
\normalfont n^r\sumt^n \frac{1}{t^{r-1}}(\mg_{t,n}(\theta))^2 = \;& g(\theta,r,m)+ o(1)\;\; \tag{\textit{i}} \\
n^{1/2}\sumt^n t^{-1/2}\mg_{t,n}(\theta) = \;& \frac{\Gamma(m+1)}{(1/2-\theta)^{m}(2\theta-1)}+ o(1), \tag{\textit{ii}} 
\end{align}
where \(g(\theta,r,m) \coloneqq r^{-2m+1}(2\theta/r-1)^{-2m-1}m(m+(2/r)(\theta/r-1)\theta)\Gamma(2m-1)\). Moreover,
\begin{align}
n\sumt^n g_{t,n}^2(\theta) = \;& \frac{\theta^2}{2\theta-1} + o(1) \tag{\textit{iii}}  \\
n\sumt^n g_{t,n}(\theta)g_{t,n} = \;& \frac{\theta\theta_0}{c_0\theta_0+\theta-1}+ o(1) \tag{\textit{iv}} \\
n\sum_{t \eq 2}^n\sumj^{t-1}g_{t,n}(\theta)g_{j,n}(\theta) g_{j,t}  = \;&  \frac{\theta^2\theta_0}{(2\theta-1)(c_0\theta_0+\theta-1)} + o(1) \tag{\textit{v}} \\
n\sum_{t \eq 2}^n\sumj^{t-1}g_{t,n}(\theta)g_{j,n} g_{j,t}  = \;&  \frac{\theta\theta_0^2}{(2c_0\theta_0-1)(c_0\theta_0+\theta-1)} + o(1) \tag{\textit{vi}} \\
n\sumt^n \dg_{t,n}g_{t,n} = \;& \frac{\theta_0(c_0\theta_0-1)}{(\theta_0(1+c_0)-1)^2}+ o(1) \tag{\textit{vii}} \\
n\sum_{t \eq 2}^n\sumj^{t-1}\dg_{t,n}g_{j,n} g_{j,t}  = \;&  \frac{\theta_0^2(c_0\theta_0-1)}{(2c_0\theta_0-1)(\theta_0(1+c_0)-1)^2} + o(1) \tag{\textit{viii}}\\
n\sum_{t \eq 2}^n\sumj^{t-1}\dg_{t,n}\dg_{j,n} g_{j,t}  = \;&  \frac{\theta_0(\theta_0(2c_0(\theta_0 - 1)\theta_0  + c_0 - \theta_0  + 2) - 1)}{(2\theta_0  - 1)^3((1+c_0)\theta_0 - 1)^2} + o(1). \tag{\textit{ix}}
\end{align}
\end{lemma}


==> nls_preliminary_old.tex <==
\subsection{Preliminaries}

\textbf{A.1.1 Working formula for \(a_n\) when  \(\{\theta_0,\fra_0\}\) are unknown.} Given the sample \(\{y_1,\dots,y_n\}\), one obtains a counterpart of Eq. \eqref{eq:AST} that holds for any \(\theta\) and any initial value \(\mathfrak{a} \in \mathbb{R}\) from the following recursive representation
\begin{equation} 
a_{n}(\theta,\fra) = a_{n-1}(\theta,\fra)  + \frac{\theta}{n}(y_n - a_{n-1}(\theta,\fra)),\quad a_0(\theta,\fra) \coloneqq \fra,
\end{equation}
 where the notation \(a_{n}(\theta,\mathfrac{a})\) is used to make the dependence on the initial value \(\mathfrak{a}\) explicit. Thus, Eq. \eqref{eq:AST} is recovered from the preceeding display by using the true parameters \(\{\theta_0,\fra_0\}\); i.e., \(a_{n}(\theta_0,\fra_0)\). Next, by adding and subtracting \(\alpha_0 = \delta_0/(1-\beta_0)\), it follows for all \(n \geq 1\) that
\begin{equation}  \label{eq:ASTgamma} 
\begin{split}
a_{n}(\theta,\fra) - \alpha_0 = \,& (a_{n-1}(\theta,\fra)-\alpha_0)\left(1-\frac{\theta}{n}\right)  + \frac{\theta}{n}(y_n - \alpha_0) \\
= \,& (a_{n-2}(\theta,\fra)-\alpha_0)\left(1-\frac{\theta}{n}\right)\left(1-\frac{\theta}{n-1}\right) \\
\,& + \frac{\theta}{n}(y_n - \alpha_0)+\left(1-\frac{\theta}{n}\right)\frac{\theta}{n-1}(y_{n-1} - \alpha_0) \\
\vdots \,& \\
a_n(\theta,\mathfrak{a})  - \alpha_0 = \,& (\mathfrak{a}-\alpha_0)\Phi_{n,1}(\theta) + \sum_{t \eq 1}^n g_{t,n}(\theta)(y_t-\alpha_0)
\end{split}
\end{equation}
for \(g_{t,n}(\theta) \coloneqq g_{t,n}(\theta,0)\), with
\[
g_{t,n}(\theta,\beta) =  \frac{\theta}{t}\Phi_{t,n+1}(\theta,\beta),\;\;\Phi_{t,n+1}(\theta,\beta) \coloneqq \prod_{j \eq t +1}^n\bigg[1-(1-\beta)\frac{\theta}{j}\bigg].
\]
As a notational convention, I set throughout \(\Phi_{n,n+1}(\theta,\beta) \coloneqq 1\), \(\Phi_{0}(\theta,\beta) \coloneqq 1\) and let \(\Phi_{n,t+1}(\theta) \coloneqq \Phi_{n,t+1}(\theta,0)\), \(\Phi_{n}(\theta,\beta) \coloneqq \Phi_{n,1}(\theta,\beta)\).  

\noindent \textbf{A.1.2 Working formula for \(a_n\) when  \(\{\theta_0,\fra_0\}\) are known.} We can rewrite Eq. \eqref{eq:ALM} as 
\begin{equation}
y_t -\alpha_0 = \beta_0a_{t-1}^\st+\eps_t, \quad a_t^\st \coloneqq a_t-\alpha_0.
\end{equation}
As shown e.g. in \citet[Appendix A]{may21}, by inserting the expression for \(y_t -\alpha_0\) from the preceding display back into Eq. \eqref{eq:ASTgamma} one arrives at
\begin{equation}
a_n^\st = (\mathfrak{a}_0-\alpha_0)\Phi_{n} + \sum_{t \eq 1}^n g_{t,n}\eps_t, \quad g_{t,n} \coloneqq g_{t,n}(\theta_0,\beta_0) = \frac{\theta_0}{t}\Phi_{n,t+1},
\end{equation}
with \(\Phi_{n,t+1} \coloneqq \Phi_{n,t+1}(\theta_0,\beta_0)\) and \(\Phi_{n} \coloneqq \Phi_{n,1}\).

\noindent \textbf{A.1.3 Effect of the initial value \(\fra\).} As shown below in Lemma \ref{lemma_aux5}, 
\[
\Ex\big[\ssupt\ssup\limits_{\fra\inn\mathbb{R}}|Q_n(\theta,\fra)-Q_n^\dagger(\theta)|\big] = O(1), 
\]
with
\[
Q_n(\theta,\fra) \coloneqq \sumt^n(z_t-a_{t-1}(\theta,\fra))^2,\quad Q_n^\dagger(\theta) \coloneqq \sumt^n(z_t-a_{t-1}^\dagger(\theta))^2,
\]
where, 
\begin{equation}\label{eq:ASTtheta}
a_n^\dagger(\theta) = \begin{cases}
\mathfrak{a}_0 & \text{if } n = 0, \\
\alpha_0 + \sum_{t \eq 1}^n  g_{t,n}(\theta)(y_t-\alpha_0) & \, \text{otherwise}.
\end{cases}
\end{equation}
Therefore, I redefine \(a_n(\theta) = a_n^\dagger(\theta)\) and work in the following with \(a_n(\theta)\) instead of \(a_n(\theta,\fra)\). For future reference, set
\[
a_n^\st(\theta) \coloneqq a_n(\theta)-\alpha_0.
\]

\noindent \textbf{A.1.4 Notational conventions.} Next, define \(\normalfont \mg_{t,n}(\theta) \coloneqq \textsf{d}^m\,g_{t,n}(\theta)/(\textsf{d}\,\theta^m)\), and similarly \(\normalfont \ma_{n}(\theta) \coloneqq \textsf{d}^m\,a_{n}(\theta)/(\textsf{d}\,\theta^m)\), \(m \in \mathbb{N}_+\). For the first four derivatives, the notation \(\dg_{t,n}(\theta)\), \(\ddot{g}_{t,n}(\theta)\), \(\dddot{g}_{t,n}(\theta)\), and \(\ddddot{g}_{t,n}(\theta)\) is used; similar for \(a_{n}(\theta)\). Finally, set \(\dg_{t,n} \coloneqq \dg_{t,n}(\theta_0)\), \(\da_n \coloneqq \da_n(\theta_0)\) and let \(c_0 \coloneqq 1-\beta_0\).


==> nls_proof_prop3.tex <==
Consistency of \(\hat{\sigma}_{n,u}^2\) is due to the fact that \(n^{-1}(Q_n(\htheta_n)-Q_n(\theta_0)) = o_p(1)\), which, in turn, follows from the proof of Proposition \ref{prop:consistency}. Turning to \(\hat{\sigma}_{n,\da}^2\), note that 
\begin{equation}
\begin{split}\nn
|h_t^2(\theta,\halpha_n)-\da_t^2(\theta)| \leq \,& (\halpha_n-\alpha_0)^2\big(\sumi^t \dg_{i,t}(\theta)\big)^2+2|\halpha_n-\alpha_0||\da_t(\theta)||\sumi^t\dg_{i,t}(\theta)|\\
\leq \,& (\halpha_n-\alpha_0)^2\big(t\sumi^t \dg_{i,t}^2(\theta)\big)+2|\halpha_n-\alpha_0||\da_t(\theta)|\big(t\sumi^t \dg_{i,t}^2(\theta)\big)^{1/2},
\end{split}
\end{equation}
where the second inequality is due to Cauchy-Schwarz. Next, since \(\{\dg_{i,t}^2(\theta)\}_{i \geq i_0}\) is decreasing for any \(\theta \in [\ubtheta,\btheta]\) for some finite \(i_0 \in \mathbb{N}_0\) depending only on \(\ubtheta\), it follows from Dini's theorem and Lemma \ref{lemma_aux1} that \(t\sumi^t \dg_{i,t}^2(\theta) = O(1)\) uniformly in \(\theta\). Next, by the same argument as in Eq. \eqref{eq:rootn} from the proof of Proposition \ref{prop:normality}, \(\ssupt n^{-1/2}\sumt^n|\da_t(\theta)| = O_p(1)\). Thus, we conclude from Lemma \ref{lemma_aux3} and \(|\halpha_n-\alpha_0| = O_p(n^{-1/2})\), that 
\(
\hat{\sigma}_{n,\da}^2 = \lni\sumt^n\da_t^2(\htheta_n) + o_p(1).
\)
The claim follows from lemma \ref{lemma_aux2} and Lemma \ref{lemma_aux3}.

